Automatically Generating Rules of Malicious Software Packages via Large Language Model

Today's security tools predominantly rely on predefined rules crafted by experts, making them poorly adapted to the emergence of software supply chain attacks. To tackle this limitation, we propose a novel tool, RuleLLM, which leverages large language models (LLMs) to automate rule generation for OSS ecosystems. RuleLLM extracts metadata and code snippets from malware as its input, producing YARA and Semgrep rules that can be directly deployed in software development. Specifically, the rule generation task involves three subtasks: crafting rules, refining rules, and aligning rules. To validate RuleLLM's effectiveness, we implemented a prototype system and conducted experiments on the dataset of 1,633 malicious packages. The results are promising that RuleLLM generated 763 rules (452 YARA and 311 Semgrep) with a precision of 85.2\% and a recall of 91.8\%, outperforming state-of-the-art (SOTA) tools and scored-based approaches. We further analyzed generated rules and proposed a rule taxonomy: 11 categories and 38 subcategories.

==> analysis.tex <==
\clearpage

\section{Rule Analysis}


===================================

Category: Common Application Rules
Detected Packages: 199 (12.19%)
Triggered Rules: 8
Average Packages per Rule: 24.88

Category: Malware Family Rules
Detected Packages: 83 (5.08%)
Triggered Rules: 10
Average Packages per Rule: 8.30

Category: Other Rules
Detected Packages: 31 (1.90%)
Triggered Rules: 7
Average Packages per Rule: 4.43

================================


 
\begin{table}[!t] 
    \caption{The category and the number of generated rule. }
    \label{tab:rule:category}
    \centering
    \begin{tabular}{  c c    }
    \toprule
    Category                    &  Number   \\
    \toprule
    Metadata Related Rules  & 125 \\
    Malicious Behavior Rules  & 170 \\
    Dependency Library Rules  & 76 \\
    Setup Code Rules  & 109 \\
    Network Related Rules  & 154 \\
    Obfuscation \& Anti-Detection Rules  & 128 \\
    Data Exfiltration Rules  & 73 \\
    Code Execution Rules  & 82 \\
    Common Application Rules  & 56 \\
    Malware Family Rules  & 14 \\
    Other Rules  & 12 \\
    \toprule 
    Total  & 452 \\ 
    \toprule   
    \end{tabular}
 %   \vspace{-0.1in}
\end{table}


Category 10: Malicious Behavior Rules (Total Rules: 19) 
Total Matches: 29
Matched Packages: 12 (0.73%)

Subcategories:

c. System Configuration Changes (Rules: 7)
   Matches: 10
   Packages: 4 (0.24%)
   Rule Files: 5

d. Persistence Mechanisms (Rules: 12)
   Matches: 19
   Packages: 10 (0.61%)
   Rule Files: 9

================================================================================
Category 11: Other Rules (Total Rules: 6)
Total Matches: 23
Matched Packages: 21 (1.29%)

Subcategories:

a. Unknown or Undetermined (Rules: 6)
   Matches: 23
   Packages: 21 (1.29%)
   Rule Files: 6

================================================================================
Category 1: Metadata Related Rules (Total Rules: 20)
Total Matches: 724
Matched Packages: 681 (41.70%)

Subcategories:

b. Version Number Deception (Rules: 3)
   Matches: 11
   Packages: 11 (0.67%)
   Rule Files: 3

c. Dependency Metadata Forgery (Rules: 3)
   Matches: 572
   Packages: 572 (35.03%)
   Rule Files: 3

d. Author Information Spoofing (Rules: 14)
   Matches: 141
   Packages: 106 (6.49%)
   Rule Files: 13

================================================================================
Category 2: Dependency Library Rules (Total Rules: 14)
Total Matches: 134
Matched Packages: 118 (7.23%)

Subcategories:

a. System Library Abuse (Rules: 3)
   Matches: 106
   Packages: 101 (6.18%)
   Rule Files: 3

b. Network Library Misuse (Rules: 7)
   Matches: 11
   Packages: 7 (0.43%)
   Rule Files: 5

c. Crypto Library Exploitation (Rules: 2)
   Matches: 10
   Packages: 10 (0.61%)
   Rule Files: 2

d. UI/Graphics Library Abuse (Rules: 2)
   Matches: 7
   Packages: 7 (0.43%)
   Rule Files: 2

================================================================================
Category 3: Setup Code Rules (Total Rules: 50)
Total Matches: 429
Matched Packages: 338 (20.70%)

Subcategories:

a. Malicious Setup Scripts (Rules: 11)
   Matches: 196
   Packages: 186 (11.39%)
   Rule Files: 11

b. Build Process Manipulation (Rules: 3)
   Matches: 6
   Packages: 6 (0.37%)
   Rule Files: 3

c. Installation Hook Abuse (Rules: 17)
   Matches: 96
   Packages: 70 (4.29%)
   Rule Files: 14

d. Package Configuration Tampering (Rules: 19)
   Matches: 131
   Packages: 104 (6.37%)
   Rule Files: 17

================================================================================
Category 4: Network Related Rules (Total Rules: 62)
Total Matches: 578
Matched Packages: 359 (21.98%)

Subcategories:

a. C2 Communication (Rules: 12)
   Matches: 48
   Packages: 30 (1.84%)
   Rule Files: 10

b. Data Exfiltration Channels (Rules: 11)
   Matches: 41
   Packages: 39 (2.39%)
   Rule Files: 8

c. Malicious Downloads (Rules: 30)
   Matches: 471
   Packages: 341 (20.88%)
   Rule Files: 22

d. DNS/Protocol Abuse (Rules: 9)
   Matches: 18
   Packages: 7 (0.43%)
   Rule Files: 6

================================================================================
Category 5: Obfuscation \& Anti-Detection Rules (Total Rules: 79)
Total Matches: 1357
Matched Packages: 1111 (68.03%)

Subcategories:

a. Code Obfuscation (Rules: 18)
   Matches: 76
   Packages: 49 (3.00%)
   Rule Files: 13

b. Anti-Analysis Techniques (Rules: 27)
   Matches: 1168
   Packages: 1094 (66.99%)
   Rule Files: 22

c. Sandbox Evasion (Rules: 9)
   Matches: 23
   Packages: 18 (1.10%)
   Rule Files: 5

d. String/Pattern Hiding (Rules: 25)
   Matches: 90
   Packages: 35 (2.14%)
   Rule Files: 17

================================================================================
Category 6: Data Exfiltration Rules (Total Rules: 57)
Total Matches: 865
Matched Packages: 462 (28.29%)

Subcategories:

a. Credential Theft (Rules: 3)
   Matches: 5
   Packages: 5 (0.31%)
   Rule Files: 2

b. Environment Data Stealing (Rules: 15)
   Matches: 70
   Packages: 50 (3.06%)
   Rule Files: 9

d. Sensitive Data Harvesting (Rules: 39)
   Matches: 790
   Packages: 457 (27.99%)
   Rule Files: 33

================================================================================
Category 7: Code Execution Rules (Total Rules: 75)
Total Matches: 1652
Matched Packages: 921 (56.40%)


Subcategories:

a. Shell Command Execution (Rules: 50)
   Matches: 1179
   Packages: 707 (43.29%)
   Rule Files: 37

b. Script Injection (Rules: 24)
   Matches: 471
   Packages: 443 (27.13%)
   Rule Files: 14

c. Process Creation (Rules: 1)
   Matches: 2
   Packages: 2 (0.12%)
   Rule Files: 1

================================================================================
Category 8: Common Application Rules (Total Rules: 56)
Total Matches: 336
Matched Packages: 199 (12.19%)

Subcategories:

a. Messaging Platform Abuse (Rules: 34)
   Matches: 235
   Packages: 189 (11.57%)
   Rule Files: 26

b. Social Media API Exploitation (Rules: 1)
   Matches: 2
   Packages: 2 (0.12%)
   Rule Files: 1

c. Cloud Service Misuse (Rules: 16)
   Matches: 90
   Packages: 72 (4.41%)
   Rule Files: 14

d. Development Tool Abuse (Rules: 5)
   Matches: 9
   Packages: 5 (0.31%)
   Rule Files: 5

================================================================================
Category 9: Malware Family Rules (Total Rules: 14)
Total Matches: 91
Matched Packages: 79 (4.84%)

Subcategories:

a. Known Trojan Families (Rules: 12)
   Matches: 85
   Packages: 75 (4.59%)
   Rule Files: 11

d. Backdoor Families (Rules: 2)
   Matches: 6
   Packages: 6 (0.37%)
   Rule Files: 2



\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{source/rule_example.pdf}
    \caption{One rule example generated by {\tech}}
    \label{fig:enter-label}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.88\linewidth]{source/rule_example.pdf}
%     \caption{ One rule example generated by {\tech} }
%     \label{fig:example}
% \end{figure}

\textbf{Case Study}.
Figure~\ref{fig:enter-label} depicts one rule example generated by {\tech}, which is used to detect a malicious script (`setup.py').
The description part is used to describe the purpose of the rule- to detect a specific setup.py script, which intends to install a software package called steembase and contains customized installation logic. 
The rule identifies socket.gethostname(), os.getcwd(), and getpass.getuser() as key indicators of malicious behavior. requests.get() is used to send HTTP requests and is also an important feature of malicious behavior.
The rule details how this information is retrieved via the ploads dictionary and passed to requests.get(), indicating a potential data leakage risk.
In short, the rules generated by {\tech} are interpretable and logical.





\begin{figure}
    \centering
    \includegraphics[width=2.4in]{figure/meta-overlap.pdf}
        \caption{Metadata rules for the overlapping degree between {\tech} and SOTA tools (SemGrep, Yara, and AppInspector). }
        \label{fig:meta:overlap}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=2.4in]{figure/code-overlap.pdf}
        \caption{Source code rules for the overlapping degree between {\tech} and SOTA tools (SemGrep, Yara, and AppInspector). }
        \label{fig:code:overlap}
\end{figure}


  
We further investigate the overlapping rules between {\tech} and SOTA tools (SemGrep, Yara, and AppInspector).
We extract the metadata and source code rules from each tool and compare them with the rules generated by {\tech}.
Specifically, the Levenshtein-distance is used to measure the similarity between rules.
Figure~\ref{fig:meta:overlap} shows the overlapping rules in metadata, and Figure~\ref{fig:code:overlap} shows the overlapping rules in the source code.
For metadata rules, the overlapping number is 125.
We observe that the overlapping rules are mainly in the rules of email, IP address, URL format, and some common dependencies, such as socket, request, ReverseShell, etc.


Despite having 5,055 rules, {\tech} shares relatively few rules with each of the other tools, suggesting it introduces a significant number of unique rules that aren't captured by existing tools. 
The limited overlap across all three tools indicates that {\tech} could be effectively combined with other tools for comprehensive coverage. Integrating {\tech} with Yara, Semgrep, or AppInspector could enhance detection robustness, potentially identifying both unique and overlapping patterns for improved security analysis.


\begin{table}[!t] 
    \caption{The source code rule generated by {\tech}. }
    \label{tab:rule:data}
    \centering
    \begin{tabular}{  c c    }
    \toprule
    Category                    &  Number   \\
    \toprule
    Hexadecimal                     & 138  \\
    Hashcode              & 24 \\
    filename     &  0 \\
    filesize    &   601 \\
    offset   &  1310 \\
    API \& Code &   77 \\
    \toprule 
    Total & 4,025 \\ 
    \toprule   
    \end{tabular}
 %   \vspace{-0.1in}
\end{table}

\textbf{Rule Characteristic}.
We first inspect the types of rules generated by {\tech}.
Table~\ref{tab:rule:data} shows the distribution of source code rules generated by {\tech} across different categories, including hexadecimal patterns, hash codes, filenames, file sizes, offsets, and API/code references. The total number of rules in this dataset is 4,025.
The large number of offset (1,310) and filesize (601) rules suggests that {\tech} prioritizes file structure characteristics, such as specific offsets or size constraints, which are often indicative of unique file types or tampering. These rules can be effective in detecting modified binaries or malicious files with structural anomalies.
With 138 rules, hexadecimal patterns are likely to target specific binary signatures, enabling the detection of precise byte sequences. This category is useful for identifying known threats or distinctive patterns commonly found in malware.
The relatively small number of API/code (77) and hash (24) rules suggests that {\tech} may emphasize static structural analysis (like offsets and sizes) over behavioral or hash-based rule generation. 
{\tech}'s rules can be complementary to tools that may rely more heavily on behavioral or hash-based detection.




\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figure/rule-type.pdf}
    \caption{The type distribution for the generated rules. }
    \label{fig:rule:type}
\end{figure}


Figure~\ref{fig:rule:type} shows the distribution of rule types generated by {\tech}.
The high number of file-related rules (1,939) indicates that {\tech} is heavily geared towards detecting file-based behaviors, such as file creation, modification, or access patterns often associated with malware or suspicious activity.
System rules (1,047) reflect a focus on system-level actions, which may include monitoring system calls, registry changes, or process activities that could indicate potential tampering or exploitation of system resources.
654 network-related rules describe network activities, like data transmission or connection patterns, which are relevant for identifying threats that involve network communications or data exfiltration.
Decode rules (493) might focus on identifying patterns in encoded or encrypted data within files or network traffic, which can help detect attempts to obscure malicious content.
This rule set provides a comprehensive approach, blending file-system analysis with network and remote operation monitoring, positioning {\tech} as an adaptable tool for a range of security contexts.


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figure/score-cdf.pdf}
    \caption{The CDF of the score for rules associated with malicious packages: malicious score, risk score, and confidence score. }
    \label{fig:score}
\end{figure}

\textbf{Rule Score}. 
We further investigate the rule score generated by {\tech}, including confidence score, malicious degree, and risk score.
Figure~\ref{fig:score} shows the distribution of the risk score for the generated rules.

As shown in Figure~\ref{fig:score}, after removing the risk score of 0, it can be seen that 30\% of the code has security risks. Specifically, if this code is incorrectly input, malicious behavior will occur. Some malicious features have low malicious and high risk, which is because the security of the code is considered and it is easy to be attacked. After analyzing all the source codes in the data set, the distribution of malicious, obfuscation, and risk is explained. Even in malicious third-party libraries, most of the code does not contain malicious features. Under the premise that the number of Python programs in the malicious third-party PyPI library is 9.5 and the median is 2, only about 20\% of the Python programs have malicious features.





Figure~\ref{fig:score}, almost all data have a confidence of more than 0.8 and judgments with full confidence account for more than 50\%. 
As shown in Figure~\ref{fig:score}, we can see that for the maliciousness distribution of malicious features, 80\% of the maliciousness scores are above 0.5. According to the definition in the prompt word, a score above 0.5 indicates that there is potential malicious behavior, there is a complete source to sink link in the code, and there is a risk of executing malicious behavior. It can be seen that the malicious features of the malicious behavior part have the same characteristics. From the CDF diagram of obfuscation, it can be seen that only about 5\% of malicious third-party libraries use uncommon language features, unnecessary dynamic execution, and misleading variables to perform malicious behaviors. Specific malicious behaviors include:
Using self-written modules with similar names to popular packages to perform malicious behaviors; using subprocess functions to call external processes during the installation of PyPI packages, and using os's fork, pipe, and other functions to create external processes.









\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figure/normalized_scores_boxplot.pdf}
    \caption{scores boxplot}
    \label{fig:enter-label}
\end{figure}



\begin{table}[!t] 
    \caption{Evaluating the Classification Performance of Rules Generated by RuleGen compared to baseline rules. }
    \label{tab:classification:performance}
    \centering
    \begin{tabular}{  l c c c c    }
    \toprule
    \textbf{Rule Type}          & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} \\
    \toprule
    RuleGen            & 86.4\%   & 72.3\%   & 71.3\%  & 82.9\%  \\
    Maliciousness  & 75.7\%   & 89.1\%   & 63.2\%  & 71.7\%  \\
    Mixedness       & 65.0\%   & 70.2\%   & 85.9\%  & 76.9\%  \\
    Anomaly        & 86.4\%   & 65.0\%   & 52.1\%  & 56.8\%  \\
    \toprule
    \end{tabular}
 %   \vspace{-0.1in}
\end{table}


\begin{table}[!t] 
    \caption{The effect of generating rules to classify malware. }
    \label{tab:malware:classification}
    \centering
    \begin{tabular}{  l c c c c    }
    \toprule
    \textbf{Rule Type}          & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} \\
    \toprule
    RuleGen Rules        & 86.4\%   & 72.3\%   & 71.3\%  & 82.9\%  \\
    Without Filtering Aggregated Rules   & 84.5\%   & 47.8\%   & 66.6\%  & 55.7\%  \\
    \toprule
    \end{tabular}
 %   \vspace{-0.1in}
\end{table}




\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figure/rules_overlap.pdf}
    \caption{overlap rules from all}
    \label{fig:enter-label}
\end{figure}
